The distribution of the dark matter in galaxies as the imprint of its Nature

The standard framework within which cosmological measurements are confronted and interpreted nowadays, called Lambda Cold Dark Matter, presents a Universe dominated by unknown forms of energy and matter. My Thesis is devoted to investigate the distribution of dark matter in galaxies and addresses the fact that the local universe-the small objects that orbit galaxies and the galaxy cores-turns out to be a marvelous laboratory for examining the nature of dark matter and the fundamental physics involved in structure formation and evolution. I develop tests, based on mass modeling of rotation curves, for the validation of dark matter models on galactic scales. These tests have been applied in analyzing the phenomenology of the cusp vs core controversy, and the phenomenon of non-Keplerian rotation curves as modification of the laws of gravity. I further investigate the properties and scaling laws of dark matter halos. My conclusion is that galactic observations provide strong imprints on the nature of dark matter.

==> chapter2.tex <==
\chapter{DM candidates, direct and indirect searches}

